Rectilinear Link Diameter and Radius in a Rectilinear Polygonal Domain

We study the computation of the diameter and radius under the rectilinear link distance within a rectilinear polygonal domain of $n$ vertices and $h$ holes. We introduce a \emph{graph of oriented distances} to encode the distance between pairs of points of the domain. This helps us transform the problem so that we can search through the candidates more efficiently. Our algorithm computes both the diameter and the radius in $\min \{\,O(n^\omega), O(n^2 + nh \log h + \chi^2)\,\}$ time, where $\omega<2.373$ denotes the matrix multiplication exponent and $\chi\in \Omega(n)\cap O(n^2)$ is the number of edges of the graph of oriented distances. We also provide a faster algorithm for computing the diameter that runs in $O(n^2 \log n)$ time.

==> metadata/acknowledgements.tex <==
\acknowledgements{}%optional


==> metadata/authorrunning.tex <==
% Mandatory. First: Use abbreviated first/middle names. Second (only in severe
% cases): Use first author plus 'et. al.'
\authorrunning{E. Arseneva \etal}


==> metadata/authors-v2018.tex <==
% Please provide for each author the \author and \affil macro, even when
% authors have the same affiliation, i.e. for each author there needs to be the
% \author and \affil macros
\def\emailkenny{chiumk@zedat.fu-berlin.de}
\def\emailandre{andre.vanrenssen@sydney.edu.au}
\def\emailmarcel{m.j.m.roeloffzen@tue.nl}
\def\emailelena{ea.arseneva@gmail.com}
\def\emailaure{aureooms@ulb.ac.be}
\def\emailmati{matias.korman@tufts.edu}
\def\emailalex{a.markovic@tue.nl}
\def\emailyoshio{okamotoy@uec.ac.jp}

\def\orcidkenny{}
\def\orcidandre{https://orcid.org/0000-0002-9294-9947}
\def\orcidmarcel{}
\def\orcidelena{https://orcid.org/0000-0002-5267-4512}
\def\orcidaure{https://orcid.org/0000-0002-5733-1383}
\def\orcidmati{}
\def\orcidalex{}
\def\orcidyoshio{https://orcid.org/0000-0002-9826-7074}

\def\affilulb{Universit\'e libre de Bruxelles (ULB), Brussels, Belgium}
\def\affiltou{Tufts University, Boston, USA}
\def\affiltue{TU Eindhoven, Eindhoven, the Netherlands}
\def\affiluec{University of Electro-Communications, Tokyo, Japan}
\def\affilaip{RIKEN Center for Advanced Intelligent Project, Tokyo, Japan}
\def\affilsyd{University of Sydney, Sydney, Australia}
\def\affilfub{Institut f\"ur Informatik, Freie Universit\"at Berlin, Berlin, Germany}
\def\affilspbu{St. Petersburg State University, St. Petersburg, Russia}

\def\supportjst{Supported by JST ERATO Grant Number JPMJER1201, Japan.}
\def\supportelena{Partially supported by the SNF Early Postdoc Mobility grant P2TIP2-168563, Switzerland, and F.R.S.-FNRS, Belgium.}
\def\supportmati{Supported in part by KAKENHI No. 17K12635, Japan and NSF award CCF-1422311.}
\def\supportalex{Supported by the Netherlands' Organisation for Scientific Research (NWO) under project no.~024.002.003.}
\def\supportyoshio{Partially supported by JSPS KAKENHI Grant Number 15K00009 and JST CREST Grant Number JPMJCR1402, and Kayamori Foundation of Informational Science Advancement.}
\def\supportaure{Supported by the Fund for Research Training in Industry and Agriculture (FRIA).}
\def\supportfub{Supported in part by ERC StG 757609.}

\author{Elena Arseneva}{\affilspbu}{\emailelena}{\orcidelena}{\supportelena}
\author{Man-Kwun Chiu$^{7,}$}{\affilfub}{\emailkenny}{\orcidkenny}{\supportfub}
\author{Matias Korman}{\affiltou}{\emailmati}{\orcidmati}{\supportmati}
\author{Aleksandar Markovic}{\affiltue}{\emailalex}{\orcidalex}{\supportalex}
\author{Yoshio Okamoto}{\affiluec\\ \affilaip}{\emailyoshio}{\orcidyoshio}{\supportyoshio}
\author{Aurélien Ooms}{\affilulb}{\emailaure}{\orcidaure}{\supportaure}
\author{Andr\'{e} van Renssen}{\affilsyd}{\emailandre}{\orcidandre}{\supportjst}
\author{Marcel Roeloffzen$^7$}{\affiltue}{\emailmarcel}{\orcidmarcel}{}


==> metadata/category.tex <==
\category{}%optional, e.g. invited paper


==> metadata/copyright.tex <==
\Copyright{Elena Arseneva, Man-Kwun Chiu, Matias Korman,  Aleksandar Markovic, Yoshio Okamoto, Aur\'elien Ooms, Andr\'{e} van Renssen, Marcel Roeloffzen}%mandatory, please use full first names. LIPIcs license is "CC-BY";  http://creativecommons.org/licenses/by/3.0/


==> metadata/editors-v2016.tex <==
%Editor-only macros:: begin (do not touch as author)%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\EventEditors{John Q. Open and Joan R. Acces}
\EventNoEds{2}
\EventLongTitle{42nd Conference on Very Important Topics (CVIT 2016)}
\EventShortTitle{CVIT 2016}
\EventAcronym{CVIT}
\EventYear{2016}
\EventDate{December 24--27, 2016}
\EventLocation{Little Whinging, United Kingdom}
\EventLogo{}
\SeriesVolume{99}
\ArticleNo{20} %
% Editor-only macros::end %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> metadata/editors-v2018.tex <==
%Editor-only macros:: begin (do not touch as author)%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\EventEditors{Wen-Lian Hsu, Der-Tsai Lee, and Chung-Shou Liao}
\EventNoEds{3}
\EventLongTitle{29th International Symposium on Algorithms and Computation (ISAAC 2018)}
\EventShortTitle{ISAAC 2018}
\EventAcronym{ISAAC}
\EventYear{2018}
\EventDate{December 16--19, 2018}
\EventLocation{Jiaoxi, Yilan, Taiwan}
\EventLogo{}
\SeriesVolume{123}
\ArticleNo{27} %%Your submission number in EasyChair(=<article-no>)
%\nolinenumbers %uncomment to disable line numbering
%\hideLIPIcs  %uncomment to remove references to LIPIcs series (logo, DOI, ...), e.g. when preparing a pre-final version to be uploaded to arXiv or another public repository
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> metadata/funding.tex <==
\funding{}%optional, to capture a funding statement, which applies to all authors. Please enter author specific funding statements as fifth argument of the \author macro.


==> metadata/keywords.tex <==
\keywords{Rectilinear link distance, polygonal domain, diameter, radius}% mandatory: Please provide 1-5 keywords


==> metadata/relatedversion.tex <==
\relatedversion{A full version %of this paper
is available at \url{https://arxiv.org/abs/1712.05538}}%optional, e.g. full version hosted on arXiv, HAL, or other respository/website


==> metadata/subjclass-v2016.tex <==
% mandatory: Please choose ACM 1998 classifications from
% http://www.acm.org/about/class/ccs98-html . E.g., cite as "F.1.1 Models of
% Computation".
\subjclass{F.2.2 Nonnumerical Algorithms and Problems}


==> metadata/subjclass-v2018.tex <==
\subjclass{%
\ccsdesc[500]{Theory of computation~Computational geometry}%
}


==> metadata/title-v2016.tex <==
\title{Rectilinear Link Diameter and Radius in a Rectilinear Polygonal Domain\footnote{
     EA was partially supported by the SNF Early Postdoc Mobility grant P2TIP2-168563, Switzerland, and F.R.S.-FNRS, Belgium.
     MC, AvR and MR were supported by JST ERATO Grant Number JPMJER1201, Japan.
     MK was supported in part by KAKENHI Nos.\ 15H02665 and 17K12635, Japan. 
     AM was supported by the Netherlands' Organisation for Scientific Research (NWO) under project no.~024.002.003.
     YO was partially supported by JSPS KAKENHI Grant Number 15K00009 and JST CREST Grant Number JPMJCR1402, and Kayamori Foundation of Informational Science Advancement.
     AO was supported by the Fund for Research Training in Industry
and Agriculture (FRIA).}
     \footnote{A full version of the paper is available at \cite{DBLP:journals/cacm/Knuth74}, \url{XXX}}}
%\titlerunning{A Sample LIPIcs Article} %optional, in case that the title is too long; the running title should fit into the top page column


==> metadata/title-v2018.tex <==
\title{Rectilinear Link Diameter and Radius in a Rectilinear Polygonal Domain}
%\titlerunning{A Sample LIPIcs Article} %optional, in case that the title is too long; the running title should fit into the top page column

